RankPrompt: Step-by-Step Comparisons Make Language Models Better Reasoners

Large Language Models (LLMs) have achieved impressive performance across various reasoning tasks. However, even state-of-the-art LLMs such as ChatGPT are prone to logical errors during their reasoning processes. Existing solutions, such as deploying task-specific verifiers or voting over multiple reasoning paths, either require extensive human annotations or fail in scenarios with inconsistent responses. To address these challenges, we introduce RankPrompt, a new prompting method that enables LLMs to self-rank their responses without additional resources. RankPrompt breaks down the ranking problem into a series of comparisons among diverse responses, leveraging the inherent capabilities of LLMs to generate chains of comparison as contextual exemplars. Our experiments across 11 arithmetic and commonsense reasoning tasks show that RankPrompt significantly enhances the reasoning performance of ChatGPT and GPT-4, with improvements of up to 13%. Moreover, RankPrompt excels in LLM-based automatic evaluations for open-ended tasks, aligning with human judgments 74% of the time in the AlpacaEval dataset. It also exhibits robustness to variations in response order and consistency. Collectively, our results validate RankPrompt as an effective method for eliciting high-quality feedback from language models.

==> tables/case_study.tex <==

\begin{table*}
    \small
    \centering
    \vspace{10pt}
    % \renewcommand{\arraystretch}{1.25}
    % \rowcolors{2}{white}{gray!15}
    
    \begin{tabular}{p{0.5\textwidth}|p{0.5\textwidth}}
        \toprule
        {\textbf{Question:} Rosie runs 6 miles per hour. She runs for 1 hour on Monday, 30 minutes on Tuesday, 1 hour on Wednesday, and 20 minutes on Thursday. If she wants to run 20 miles for the week, how many minutes should she run on Friday?} & {\textbf{Question:} Each bird eats 12 beetles per day, each snake eats 3 birds per day, and each jaguar eats 5 snakes per day. If there are 6 jaguars in a forest, how many beetles are eaten each day?} \\
        \midrule
        {\textbf{Answer 1:} By the end of Thursday, she has run a total of 6 + 3 + 6 + 2 = 17 miles. To reach her goal of 20 miles for the week, she needs to run an additional 20 - 17 = 3 miles. Since she runs at a speed of 6 miles per hour, she can run 1 mile in 10 minutes. Therefore, she needs to run for 3 * 10 = 30 minutes on Friday. The answer is 30.\ding{52}} & {\textbf{Answer 1:} The total number of beetles eaten by all the birds is 12 x total number of birds. \textcolor{red}{Since each snake eats 3 birds per day, the total number of birds is the same as the total number of snakes killed by the jaguars. So, the total number of birds is 3 x 6 = 18.} So, the total number of beetles eaten each day is 12 x 18 = 216. The answer is 216.\ding{56}} \\

        {\textbf{Answer 2:} In total, Rosie runs 6 miles/hour x 1 hour/day x 4 days = 24 miles for the week from Monday to Thursday. \textcolor{blue}{To reach her goal of running 20 miles, she needs to run 20 - 24 = -4 more miles.} Since it is impossible to run negative miles, Rosie has already exceeded her goal. The answer is 0.\ding{56}} & {\textbf{Answer 2:} Each jaguar would be eating 3 x 5 = 15 birds per day. The total number of birds eaten each day would be 6 x 15 = 90. \textcolor{red}{Since each bird eats 12 beetles per day, then the total number of beetles eaten each day would be 90 x 12 = 1080}. Therefore, 1080 beetles are eaten each day. The answer is 1080.\ding{52}}  \\
        
        {\textbf{Answer 3:} In total, Rosie runs for 1 hour + 30 minutes + 1 hour + 20 minutes = 2 hours 50 minutes = 170 minutes. At 6 miles per hour, she runs 6 * 60 = 360 minutes per mile. So Rosie needs to run a total of 20 * 360 = 7200 minutes for the week. \textcolor{blue}{She has already run for 170 minutes, so she needs to run for a total of 7200 - 170 = 7030 minutes for the week.} On Friday, she has one day left to run, so she needs to run for 7030 / 480 = 14.6 minutes, which is approximately 15 minutes. The answer is 15.\ding{56}} &
        {\textbf{Answer 3:} \textcolor{red}{Each bird eats 12 beetles per day, so 6 birds eat 6 x 12 = 72 beetles per day.} Each snake eats 3 birds per day, so 6 snakes eat 6 x 3 = 18 birds per day. Each jaguar eats 5 snakes per day, so 6 jaguars eat 6 x 5 = 30 snakes per day. Therefore, the total number of beetles eaten each day is 72 x 6 = 432. The answer is 432.\ding{56}} \\
        
        \midrule
        {\textbf{Comparison:} Answer 1 correctly calculate the total distance Rosie runs from Monday to Thursday as 17 miles. Answer 1 correctly calculates the time Rosie needs to run on Friday as 30 minutes. \textcolor{blue}{Answer 2 incorrectly calculates the total distance Rosie runs from Monday to Thursday as 24 miles.} Answer 2 incorrectly calculates the remaining distance Rosie needs to run as -4 miles. Answer 2 incorrectly states that Rosie does not need to run on Friday. \textcolor{blue}{Answer 3 incorrectly calculates the total time Rosie needs to run for the week as 7030 minutes.} Answer 3 incorrectly calculates the time Rosie needs to run on Friday as 14.6 minutes, which is then rounded up to 15 minutes.} & {\textbf{Comparison:}
        Answer 1 and Answer 2 correctly calculate the total number of birds eaten by all the snakes and jaguars. Answer 3 calculates the number of birds, snakes, and jaguars separately. \textcolor{red}{Answer 1 correctly calculates the total number of beetles eaten by all the birds. Answer 2 and Answer 3 incorrectly assume that each jaguar eats all the birds killed by the snakes.}} \\
        
        {\textbf{Conclusion:} The final answer is 30 minutes.\textcolor{green}{\ding{52}}} &
        {\textbf{Conclusion:} The final answer is 216 beetles eaten each day.\textcolor{red}{\ding{56}}} \\

        \bottomrule
    \end{tabular}
    % \vspace{-10pt}
    \caption{The comparison between correct prompt and incorrect prompt generated by ChatGPT (\texttt{gpt-3.5-turbo}).}
    \label{tab:case_study}
\end{table*}
